GRAM: Global Reasoning for Multi-Page VQA

The increasing use of transformer-based large language models brings forward the challenge of processing long sequences. In document visual question answering (DocVQA), leading methods focus on the single-page setting, while documents can span hundreds of pages. We present GRAM, a method that seamlessly extends pre-trained single-page models to the multi-page setting, without requiring computationally-heavy pretraining. To do so, we leverage a single-page encoder for local page-level understanding, and enhance it with document-level designated layers and learnable tokens, facilitating the flow of information across pages for global reasoning. To enforce our model to utilize the newly introduced document tokens, we propose a tailored bias adaptation method. For additional computational savings during decoding, we introduce an optional compression stage using our compression-transformer (C-Former),reducing the encoded sequence length, thereby allowing a tradeoff between quality and latency. Extensive experiments showcase GRAM's state-of-the-art performance on the benchmarks for multi-page DocVQA, demonstrating the effectiveness of our approach.

==> Tables/MPDocVQA_DUDE_compressed.tex <==
\begin{table*}[ht]
  \centering
  \bgroup
  \def\arraystretch{1.1}
  \resizebox{1\linewidth}{!}{%
  \begin{tabular}{l c | c | c c c c c}
    \toprule
    \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{Params}} & \multicolumn{1}{c}{\textbf{MPDocVQA}} & \multicolumn{5}{c}{\textbf{DUDE}} \\
    % \cmidrule(lr){3-3}\cmidrule(lr){4-8}
    & & \multirow{2}{*}{\textbf{ANLS}}  & \multirow{2}{*}{\textbf{ANLS}} & \multicolumn{4}{c}{\textbf{ANLS per Question Type}} \\
    & & & & Extractive & Abstractive & List of answers & Unanswerable \\
    \hline
    \rowcolor{golden!20} $\text{GRAM}_{compressed}$ & $286M$ & $62.98$ & $24.25$ & $12.36$ & $21.03$ & $5.08$ & $55.75$  \\

    % large models
    \hline
    \rowcolor{golden!20} $\text{GRAM}_{compressed}$  & $859M$ & $73.37$ & $34.41$ & $23.99$ & $31.65$ & $7.55$ & $65.86$  \\ 	

    % training with both MPDocVQA + DUDE
    \hline
    \rowcolor{golden!20} $\text{GRAM}_{compressed}^\dagger$ & $859M$ & $73.80$ & $49.14$ & $50.70$ & $48.20$ & $15.35$ & $631.4$ \\
    

    \bottomrule
    
  \end{tabular}
  }
  \egroup
  \caption{}
  \label{table:MPDocVQA_DUDE_comp}
\end{table*}

==> Tables/rebuttal_ablation.tex <==
% \tabcolsep=0.09cm
% \begin{table}[]
%   \centering
%   \bgroup
%   \def\arraystretch{1.1}
%   \resizebox{1\linewidth}{!}{
%   \begin{tabular}{c c | c c c c c}
%     \toprule
%         {\textbf{Division}} & {\textbf{Page}} & \multicolumn{5}{c}{\textbf{ANLS by Number of Pages}} \\
%         & {\textbf{Embedding}} & \multicolumn{5}{c}{\textbf{DUDE validation dataset}} \\
%         & & All & 1 & 2-4 & 5-10 & 11-end \\
%             \hline

%             page & \cmark & $\mathbf{47.88}$ & $\mathbf{49.29}$ & $\mathbf{49.90}$ & $\mathbf{45.90}$ & $\mathbf{43.94}$ \\

%             \hline
%              page & \xmark & $46.12$ & $48.74$ & $48.11$ & $43.59$ & $40.99$ \\
%             \hline
%              % 128 tokens & \cmark & $44.79$ & $45.17$ & $45.22$ & $44.05$ & $\mathbf{44.11}$ \\
%              256 tokens & \cmark & $45.22$ & $46.38$ & $46.69$ & $44.13$ & $41.83$ \\
%              512 tokens & \cmark & $45.09$ & $45.90$ & $47.32$ & $42.65$ & $41.98$ \\
%              1024 tokens & \cmark & $44.39$ & $44.98$ & $46.63$ & $41.69$ & $41.78$ \\

%     \bottomrule
%   \end{tabular}
%   }
%   \egroup
%   \caption{Page Division Ablation Study}
%   \label{table:page_ablation}
%   % \vspace{-0.7cm}
% \end{table}

% \tabcolsep=0.09cm
% \begin{table}[]
%   \centering
%   \bgroup
%   \def\arraystretch{1.1}
%   \resizebox{1\linewidth}{!}{
%   \begin{tabular}{l | c c | c c c}
%     \toprule
%     {\textbf{Segment Method}} & page & page & 256 tokens & 512 tokens & 1024 tokens\\
%     \hline
%     {\textbf{Page Embedding}} & \cmark & \xmark & \cmark & \cmark & \cmark \\
%     \hline
%     {\textbf{DUDE ANLS}} & $\mathbf{47.88}$ & $46.12$ & $45.22$ & $45.09$ & $44.39$\\
%     \bottomrule
%   \end{tabular}
%   }
%   \egroup
%   \caption{Document Segmentation Ablation Study}
%   \label{table:page_ablation}
%   % \vspace{-0.7cm}
% \end{table}



\tabcolsep=0.09cm
\begin{table}[]
  \centering
  \bgroup
  \def\arraystretch{1.1}
  \resizebox{1\linewidth}{!}{
  \begin{tabular}{l c c | c c c c c}
    \toprule
        \multirow{3}{*}{\textbf{\shortstack{Method}}} & \multirow{3}{*}{\textbf{\shortstack{Division\\ Type}}} & \multirow{3}{*}{\textbf{\shortstack{Page \\ Embedding}}} & \multicolumn{5}{c}{\textbf{ANLS by Number of Pages}} \\
        & & & \multicolumn{5}{c}{\textbf{DUDE validation dataset}} \\
        & & & All & 1 & 2-4 & 5-10 & 11-end \\
            \hline
            \multirow{5}{*}{GRAM} & \rowcolor{golden!20} \multirow{1}{*}{page} & \cmark & $\mathbf{47.88}$ & $\mathbf{49.29}$ & $\mathbf{49.90}$ & $\mathbf{45.90}$ & $\mathbf{43.94}$ \\
             & \multirow{1}{*}{page} & \xmark & $46.12$ & $48.74$ & $48.11$ & $43.59$ & $40.99$ \\
             & 256 tokens & \cmark & $45.22$ & $46.38$ & $46.69$ & $44.13$ & $41.83$ \\
             & 512 tokens & \cmark & $45.09$ & $45.90$ & $47.32$ & $42.65$ & $41.98$ \\
             & 1024 tokens & \cmark & $44.39$ & $44.98$ & $46.63$ & $41.69$ & $41.78$ \\

            \hline
            % \multicolumn{2}{l}{Longformer [35]}  & \cmark & $27.14$ & - & - & - & - \\
            \multicolumn{2}{l}{$\text{DocFormerV2}_{\text{concat}}$}  & \cmark & $44.32$ & $46.08$ & $47.05$ & $42.81$ & $38.17$ \\
            \multicolumn{2}{l}{$\text{DocFormerV2}_{\text{Longformer}}$} & \cmark & $45.88$ & $47.01$ & $47.75$ & $43.22$ & $43.13$ \\
            \multicolumn{2}{l}{$\text{DocFormerV2}_{\text{AliBi}}$}& \cmark & $34.73$ & $36.55$ & $37.00$ & $30.99$ & $31.25$ \\
    \bottomrule
  \end{tabular}
  }
  \egroup
  \caption{Division method and comparison to NLP approaches}
  \label{table:rebuttal_ablation}
  \vspace{-0.3cm}
\end{table}
